SP-Allreduce: Symmetric Tree Schedules for Tori and Beyond

Allreduce is a fundamental communication primitive in large-scale distributed training, and torus interconnects remain widely deployed in high-performance systems. We introduce SP-allreduce, a new allreduce algorithm for $d$-dimensional tori that exploits the symmetry of the topology and routes only along shortest paths. We call an allreduce algorithm \emph{fully bandwidth-optimal} if it incurs no bandwidth overhead, no multihop-induced traffic inflation, and achieves perfect per-round load balance. SP-allreduce is based on a family of carefully symmetrized shortest-path trees that guarantees full bandwidth optimality in the $\alpha$--$\beta$ model. We prove that it uses the minimum possible number of rounds among all fully bandwidth-optimal allreduce algorithms on $d$-dimensional tori, and therefore the minimum running time in this class. In this sense, SP-allreduce refines Bucket allreduce: it preserves Bucket's key strengths while reducing the number of rounds by a factor of two. We further extend our approach to broader symmetric topologies and to communication trees of prescribed depths. Experimentally, the resulting algorithms improve over the best compared state-of-the-art algorithms for tori by up to $1.19\times$ on square tori and $1.65\times$ on rectangular tori across the tested configurations. On HyperX and spine-leaf networks, we demonstrate gains of up to $14.82\times$ and $1.72\times$, respectively, over the best evaluated baselines.

==> tikz_pictures.tex <==
\newcommand{\tikzPictureProofOFLemma}{
    \begin{figure}[h]
      \centering
    \begin{tikzpicture}[scale=0.3]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,9}
    \foreach \y in {1,...,9}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,8}
    \foreach \y in {1,...,8}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,...,18}{
                \draw (\x,2) to[out=150, in=30] (\x,18);
                \draw (2,\x) to[out=-60, in=60] (18,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    \foreach \x in {1,...,5}
    \foreach \y in {6,...,9}
    {
            \draw[magenta,-{Stealth[scale = 1.2]},very thick]
            (2*\x,2*\y)  -- (2*\x,2*\y-2);
    }
    \foreach \y in {1,...,4}
    \foreach \x in {5,...,9}
    {%\foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[magenta,-{Stealth[scale = 1.2]},very thick]
            (2*\x,2*\y)  -- (2*\x,2*\y+2);
    }
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,5}
    {%\foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[blue,-{Stealth[scale = 1.2]},very thick]
            (2*\x,2*\y)  -- (2*\x+2,2*\y);
    }
    \foreach \x in {6,...,9}
    \foreach \y in {5,...,9}
    {%\foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[blue,-{Stealth[scale = 1.2]},very thick]
            (2*\x,2*\y)  -- (2*\x-2,2*\y);
    }
    \end{tikzpicture}
      \caption{The tree $T_0$ for the  2D-torus of size $9\times 9$. It uses the same number of links in each direction at each stage.  The colors are for convenience.}\label{fig:PictureProofOFLemma}
    \end{figure}
}



\newcommand{\tikzPictureGatheringScattering}{
    \begin{figure}[h]
    \begin{multicols}{2}
    \begin{tikzpicture}[scale=0.7]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (6,6);
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,2)  -- (2,2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,4)  -- (10,2);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,10)  -- (10,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,8)  -- (2,10);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.7]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,{Stealth[scale = 1.2]}-,very thick]
            (\x,\y)  -- (6,6);
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (4,2)  -- (2,2);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (10,4)  -- (10,2);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (8,10)  -- (10,10);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (2,8)  -- (2,10);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}\label{fig1}
    \caption{Trees $T_g$ and $T_s$ that illustrate gathering at $(0,0)$ and then scattering the sum for the part of the vector assigned to $(0,0)$. Different arrow colors illustrate the alternating stages.}
    \end{figure}
}

\newcommand{\tikzPictureGatherScatterAnother}{
    \begin{figure}
    \begin{multicols}{4}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,2)  -- (2,2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,4)  -- (10,2);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,10)  -- (10,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,8)  -- (2,10);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (6,6);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}
    \begin{multicols}{4}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,{Stealth[scale = 1.2]}-,very thick]
            (\x,\y)  -- (6,6);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (4,2)  -- (2,2);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (10,4)  -- (10,2);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (8,10)  -- (10,10);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (2,8)  -- (2,10);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}
      \caption{The stages of gather (first line) and scatter (second line)}\label{fig2}
    \end{figure}
    
    \begin{figure}
    \begin{multicols}{2}
    \begin{tikzpicture}[scale=0.7]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (4,4);
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-4},{\y-\x+4});
    %     \draw[blue,{Stealth[scale = 1.2]}-,very thick]
    %    (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,6)  -- (4,8);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,4)  -- (8,4);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
    (4,2) to[out=150, in=30] (4,10);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
     (2,4) to[out=-60, in=60] (10,4);
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
    (2,2) to[out=150, in=30] (2,10);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
     (2,2) to[out=-60, in=60] (10,2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
    (6,2) to[out=150, in=30] (6,10);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
     (2,6) to[out=-60, in=60] (10,6);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,6)  -- (6,8);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,6)  -- (8,6);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,2)  -- (8,2);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (2,6)  -- (2,8);
    
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,10)  to[out=-60, in=60]  (10,10);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,2)  to[out=150, in=30] (8,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,8)  -- (8,8);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,6)  -- (10,8);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.7]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
            \draw[red,{Stealth[scale = 1.2]}-,very thick]
            (\x,\y)  -- (4,4);
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (\x,\y)  -- ({\x+\y-4},{\y-\x+4});
    %     \draw[blue,{Stealth[scale = 1.2]}-,very thick]
    %    (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (4,6)  -- (4,8);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (6,4)  -- (8,4);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
    (4,2) to[out=150, in=30] (4,10);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
     (2,4) to[out=-60, in=60] (10,4);
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
       \draw[red,-{Stealth[scale = 1.2]},very thick]
    (2,2) to[out=150, in=30] (2,10);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
     (2,2) to[out=-60, in=60] (10,2);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
    (6,2) to[out=150, in=30] (6,10);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
     (2,6) to[out=-60, in=60] (10,6);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
        (6,6)  -- (6,8);
         \draw[red,-{Stealth[scale = 1.2]},very thick]
        (6,6)  -- (8,6);
       \draw[red,-{Stealth[scale = 1.2]},very thick]
        (6,2)  -- (8,2);
         \draw[red,-{Stealth[scale = 1.2]},very thick]
        (2,6)  -- (2,8);
    
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (2,10)  to[out=-60, in=60]  (10,10);
       \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (8,2)  to[out=150, in=30] (8,10);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (6,8)  -- (8,8);
        \draw[blue,-{Stealth[scale = 1.2]},very thick]
        (10,6)  -- (10,8);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    \end{multicols}
    \caption{Gather/scatter for another part of the vector, collected at $(a,b)$. The original tree is translated.}
    \end{figure}
}
\newcommand{\tikzPictureTheStagesOfGather}{
    \begin{figure}
    
    \begin{multicols}{4}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,10)  to[out=-60, in=60]  (10,10);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,2)  to[out=150, in=30] (8,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,8)  -- (8,8);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,6)  -- (10,8);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
    (2,2) to[out=150, in=30] (2,10);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
     (2,2) to[out=-60, in=60] (10,2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
    (6,2) to[out=150, in=30] (6,10);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
     (2,6) to[out=-60, in=60] (10,6);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,6)  -- (6,8);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,6)  -- (8,6);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (6,2)  -- (8,2);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (2,6)  -- (2,8);
    
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-4},{\y-\x+4});
    %     \draw[blue,{Stealth[scale = 1.2]}-,very thick]
    %    (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,6)  -- (4,8);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,4)  -- (8,4);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
    (4,2) to[out=150, in=30] (4,10);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
     (2,4) to[out=-60, in=60] (10,4);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {2/4, 6/4, 4/2, 4/6}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (4,4);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (4.7,4.3) {$(a,b)$};
    
    \end{tikzpicture}
    \end{multicols}
    \begin{multicols}{4}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,2)  -- (2,2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,4)  -- (10,2);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,10)  -- (10,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,8)  -- (2,10);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.36]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10}{
                \draw (\x,2) to[out=150, in=30] (\x,10);
                \draw (2,\x) to[out=-60, in=60] (10,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (6,6);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}
      \caption{The stages of gather for $(a,b)$, next to stages for $(0,0)$. Scatter is analogous}
    \end{figure}
}

\newcommand{\tikzPictureGatherForTheEvenSizedTorus}{
    \begin{figure}
    \begin{tikzpicture}[scale=0.7]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (6,6);
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
       \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (6,10)  -- (6,12);
         \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (10,6)  -- (12,6);
       \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (6,2)  to[out=150, in=30] (6,12);
         \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (2,6)  to[out=-60, in=60] (12,6);
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,2)  -- (2,2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,4)  -- (10,2);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,10)  -- (10,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,8)  -- (2,10);
    
      \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,12)  -- (8,12);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,12)  -- (4,12);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (12,6)  -- (12,8);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (12,6)  -- (12,4);
    
    %%%%%%%%%%%%----------------------Arrows d5----------------------
    
    
      \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (8,12)  -- (10,12);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (4,12)  -- (2,12);
        \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (12,8)  -- (12,10);
        \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (12,4)  -- (12,2);
    
    %%%%%%%%%%%%----------------------Arrows d6----------------------
    
    
      \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (10,12)  -- (12,12);
       \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (2,12)  to[out=-60, in=60] (12,12);
        \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (12,10)  -- (12,12);
        \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (12,2)   to[out=150, in=30] (12,12);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \caption{Gather at $(0,0)$ for the even-sized torus. Here, dashed arrows indicate that the part of the vector that has to be gathered at $(0,0)$ is additionally split into two or four equal parts, and each part sent along one of the (two or four) dashed links going out of the vertex.}
    \end{figure}
}
\newcommand{\tikzPictureTheStagesOfGatherForTheEvenSizedTorus}{
    \begin{figure}
    \begin{multicols}{3}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d6----------------------
    
    
      \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (10,12)  -- (12,12);
       \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (2,12)  to[out=-60, in=60] (12,12);
        \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (12,10)  -- (12,12);
        \draw[blue,dashed,{Stealth[scale = 1.2]}-,very thick]
        (12,2)   to[out=150, in=30] (12,12);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d5----------------------
    
    
      \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (8,12)  -- (10,12);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (4,12)  -- (2,12);
        \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (12,8)  -- (12,10);
        \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (12,4)  -- (12,2);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d4----------------------
    
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (4,2)  -- (2,2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (10,4)  -- (10,2);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (8,10)  -- (10,10);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (2,8)  -- (2,10);
    
      \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,12)  -- (8,12);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (6,12)  -- (4,12);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (12,6)  -- (12,8);
        \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (12,6)  -- (12,4);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}
    \begin{multicols}{3}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d3----------------------
    
    \foreach \x/\y in {4/4, 8/8, 8/4, 4/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},\y);
         \draw[red,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- (\x,{2*\y-6});
    };
       \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (6,10)  -- (6,12);
         \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (10,6)  -- (12,6);
       \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (6,2)  to[out=150, in=30] (6,12);
         \draw[red,dashed,{Stealth[scale = 1.2]}-,very thick]
        (2,6)  to[out=-60, in=60] (12,6);
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    
    %%%%%%%%%%%%----------------------Arrows d2----------------------
    
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
    {%   \draw[blue,{Stealth[scale = 1.2]}-,{Stealth[scale = 1.2]}-,very thick]
     %   (\x,\y)  -- (\x,\y+2);
       \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({\x+\y-6},{\y-\x+6});
         \draw[blue,{Stealth[scale = 1.2]}-,very thick]
        (\x,\y)  -- ({2*\x-6},{2*\y-6});
    };
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \begin{tikzpicture}[scale=0.4]
    
    %%%%%%%%%%%%----------------------NODES----------------------------------
    \foreach \x in {1,...,6}
    \foreach \y in {1,...,6}
    \node at (2*\x,2*\y) {$\bullet$};
    
    %%%%%%%%%%%%----------------------EDGES----------------------------------
    \foreach \x in {1,...,5}
    \foreach \y in {1,...,5}
    \draw  (2*\x,2*\y+2) -- (2*\x,2*\y) -- (2*\x+2,2*\y) -- (2*\x+2,2*\y+2) -- cycle;
    \foreach \x in {2,4,6,8,10,12}{
                \draw (\x,2) to[out=150, in=30] (\x,12);
                \draw (2,\x) to[out=-60, in=60] (12,\x);
    
                };
    %%%%%%%%%%%%----------------------Arrows d1----------------------
    %\foreach \x in {1,...,5}
    %\foreach \y in {1,...,5}
    \foreach \x/\y in {4/6, 8/6, 6/4, 6/8}
            \draw[red,-{Stealth[scale = 1.2]},very thick]
            (\x,\y)  -- (6,6);
    
    
    %%%%%%%%%%%%----------------------Text----------------------
    
    \node at (6.7,6.3) {$(0,0)$};
    
    \end{tikzpicture}
    \end{multicols}
      \caption{The stages of gather for the even-sized torus}
    \end{figure}
}
\newcommand{\tikzPictureXXXZZZ}{

}
\newcommand{\tikzPictureXXXZZZZ}{

}
